IRIS-HEP Strategic Plan for the Next Phase of Software Upgrades for HL-LHC Physics

The quest to understand the fundamental building blocks of nature and their interactions is one of the oldest and most ambitious of human scientific endeavors. CERN's Large Hadron Collider (LHC) represents a huge step forward in this quest. The discovery of the Higgs boson, the observation of exceedingly rare decays of $B$ mesons, and stringent constraints on many viable theories of physics beyond the Standard Model (SM) demonstrate the great scientific value of the LHC physics program. The next phase of this global scientific project will be the High-Luminosity LHC (HL-LHC) which will collect data starting circa 2029 and continue through the 2030s. The primary science goal is to search for physics beyond the SM and, should it be discovered, to study its implications. In the HL-LHC era, the ATLAS and CMS experiments will record around 100 times as many collisions as were used to discover the Higgs boson (and at twice the energy). Both NSF and DOE are making large detector upgrade investments so the HL-LHC can operate in this high-rate environment. Similar investment in software R&D for acquiring, managing, processing and analyzing HL-LHC data is critical to maximize the return-on-investment in the upgraded accelerator and detectors. This report presents a strategic plan for a possible second 5-year funded phase (2023 through 2028) for the Institute for Research and Innovation in Software for High Energy Physics (IRIS-HEP) which will close remaining software and computing gaps to deliver HL-LHC science.

==> 006-old-executive-summary.tex <==
\section*{Executive Summary (Previous Version)}
\thispagestyle{empty}

The quest to understand the fundamental building blocks of nature
and their interactions is one of the oldest and most ambitious of
human scientific endeavors. CERN's Large Hadron
Collider (LHC) represents a huge step forward in this quest.  The
discovery of the Higgs boson, the observation of exceedingly rare
decays of $B$ mesons, and stringent constraints on many viable
theories of physics beyond the Standard Model (SM) demonstrate the
great scientific value of the LHC physics program. The next phase
of this global scientific project will be the High-Luminosity LHC
(HL-LHC) which will collect data starting circa 2029 and continue
through the 2030s.  The primary science goal is to search for physics
beyond the SM and, should it be discovered, to study its 
implications.  In the HL-LHC era, the ATLAS and CMS experiments
will record ${\sim}100$ times as many collisions as were used to
discover the Higgs boson (and at twice the energy). Both NSF and DOE 
are making large detector upgrade investments so the HL-LHC can
operate in this high-rate environment.  Similar investment in {\em software}
R\&D for acquiring, managing, processing and analyzing
HL-LHC data is critical to maximize the return-on-investment in the
upgraded accelerator and detectors.

This report presents a strategic plan for a possible second 
5-year funded phase (2023 through 2028) for the {\bf Institute for Research
and Innovation in Software 
for High Energy Physics (IRIS-HEP)}~\cite{iris-hep,iris-hep-nsf-award}
which will close remaining software and computing gaps to deliver HL-LHC
science.
IRIS-HEP was originally funded by the NSF in September 2018 and its 
current funding extends through August 2023. IRIS-HEP was the result 
of an international
community planning process in 2016-2017 that prepared a roadmap for
HEP software R\&D in the 2020s~\cite{CWPDOC} as well as the original
strategic plan~\cite{S2I2HEPSP} for how an NSF-funded Software
Institute for High Energy Physics (HEP) could play a key role in
meeting HL-LHC challenges. 
The mission of IRIS-HEP is two-fold: to serve as 
an active center for software R\&D {\em and} as an intellectual hub for 
the larger community software R\&D effort required to ensure the success of the HL-LHC
scientific program. 
Building on its successes over the past 5 years, IRIS-HEP will continue to
pursue several high-impact R\&D areas identified as those required to 
close the gap and enable HL-LHC science:
(1)~development of advanced innovative algorithms for data reconstruction 
and triggering; (2)~development of highly performant analysis systems that 
reduce `time-to-insight' and maximize the HL-LHC physics potential;
(3)~development of data organization, management and access systems
for the Exabyte era; and (4)~facilities R\&D to support the evolving 
requirements of the other R\&D areas. A potentially important emerging 
opportunity, (5) Translational AI, has also been identified. 
IRIS-HEP will sustain the investments
in the fabric for (6) distributed high-throughput computing which provides the LHC community's cyberinfrastructure with a route to the HL-LHC.

As an intellectual hub, the Institute will continue to lead efforts 
to (1) bring together the IRIS-HEP team, key stakeholders and relevant domain experts 
to inform the Institute’s mission, (2) bring together U.S.\ and international R\&D efforts 
in ``blueprint'' workshops to ensure full alignment of the various efforts (3) develop partnerships between HEP and the cyberinfrastructure,
computer science, and data science communities for novel approaches to
meeting HL-LHC challenges, (4) bring in new effort from U.S.\
universities emphasizing professional development and training, and
(5) sustain HEP software and underlying algorithmic and implementation
knowledge over the two decades required.
HEP is a global, complex, scientific endeavor.  These activities
will ensure that the software developed and deployed by a
globally distributed community will extend the science reach of the
HL-LHC and will be sustained over its lifetime.

The strategic plan targeting HL-LHC physics presented in this report 
for the period 2023-2028 reflects a community vision.  It 
builds on the original planning
activities in 2016-2017 and is informed by ongoing IRIS-HEP 
activities which engage the community including a dedicated series of 
workshops and conferences over the past years.
IRIS-HEP is ready to deliver the software required to enable best possible HL-LHC science. 

%Exabyte scale problems in big science.


\newpage


==> 106-strategic-areas-update-example.tex <==
\subsection{Example Focus Area}

% A general overview of the area
% Directions:
%   - Broad overview of the area - why is it important / relevant to the 
%     HL-LHC?  What part of the 4 HL-LHC challenges that we defined does 
%     this area overlap with?
%
% For reference, we defined the challenges to be:
%
% 1) Raw resource considerations (CPU, storage) needed, with a flat 
%     funding model
% 2) Scalability of the overall distributed computing cyberinfrastructure 
%    and its components 
% 3) Analysis at scale with the HL-LHC data volume/rate and complexity 
%    (user-centric)
% 4) Sustainability of the system through the science lifetime of the HL-LHC
%
% Feel free to refer back to them by name (C1, C2, …) in the text.


\subsubsection{Specific Challenges and Opportunities}
% Directions:
%  - What are the challenges specific to this area and remaining gaps
%    to the HL-LHC?  e.g. for DOMA, this might be the outright scale of
%    data transfers needed and completing the corresponding technology
%    transitions.
%  - What new things are occurring in this area that an institute-scale 
%    project could take advantage of?  Recall the timeline for us to do 
%    HL-LHC R\&D work roughly falls in the next 5 year period: there’s 
%    going to be a greater emphasis on sustainability and the later stages 
%    of the pipeline during a future institute.  We don’t need to be 
%    overly heavy on brand new threads of work.


\subsubsection{Current Approaches and Development Roadmap}
% Directions:
%  - Enumerate the list of current investments both in IRIS-HEP and around 
%    the community, as well as (clearly separated) plans for new 
%    opportunities. For each give an idea of the required development
%    directions/activities in the coming years.


\subsubsection{Impact and Success Criteria}
% Directions:
%  - What are the expected outcomes of a 5 year investment in this area?
%  - What’s the impact against the 4 HL-LHC challenges?
%  - Why is there value in US / university leadership in this area?
%  - What are potential milestones to be evaluated over the next 1-3 years 
%    post-IRIS-HEP?
%  - What are metrics for success?





==> 304-translational-ai-grand-challenge.tex <==
\subsection{Translational AI}
\label{sec:ai-grand-challenge}

Perhaps can be removed from metrics in favor of a more ``process-oriented'' approach.

\tempnewpage


==> 310-metrics.tex <==
\section{Metrics for Success - Community and Sustainability}
\label{sec:metrics}

\tempnewpage


==> 830-hep-community.tex <==
\section{Appendix - The HEP Community \textcolor{red}{30\% - REFRESH OR DROP}}

HEP is a global science. The global nature of the community is both
the context and the source of challenges for an \s2i2. A fundamental
characteristic of this community is its globally distributed knowledge
and workforce. The LHC collaborations each comprise thousands of
scientists from close to 200 institutions across more than 40
countries. The large size of these collaborations is due to the complexity of the
scientific endeavor. No one person or small team understands all aspects of
the experimental program. Knowledge is thus collectively obtained,
held, and sustained over the decades long LHC program. Much of that
knowledge is curated in software. Tens of millions of lines of code
are maintained by many hundreds of physicists and engineers.  Software
sustainability is fundamental to the knowledge sustainability
required for a research program that is expected to last 
well into the 2040s.

\subsection{The HEP Software Ecosystem and Computing Environment}

%The HEP software landscape itself is quite varied. As noted
%earlier, the software ecosystem contains elements ranging from 
%traditional ``application'' software (that could be used in the 
%context of a single workstation) to ``infrastructure'' software
%elements supporting execution of data-intensive applications on large 
%high-throughput and globally distributed computing systems. 

The HEP software landscape itself is quite varied.  Each HEP
experiment requires, at a minimum, ``application'' software for
data acquisition, data handling, data processing, simulation and
analysis, as well as related application frameworks, data persistence
and libraries.  In addition significant ``infrastructure'' software
that spans all aspects of an experiment
is required. The scale of the computing environment itself drives
some of the complexity and requirements for infrastructure tools.
Over the past 20 years, HEP experiments have became large enough 
to require significantly greater resources than the host laboratory can
provide by itself. Collaborating funding agencies typically provide 
in-kind contributions of computing resources rather than send funding
to the host laboratory. This makes a distributed computing infrastructure 
essential, and 
thus HEP research needs have driven the development of sophisticated software
for data management, data access, and workload/workflow management.

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.96\textwidth]{images/WLCG-numbers-2022.png}
\caption{The Worldwide LHC Computing Grid (WLCG), which federates national grid infrastructures to provide the computing
resources needed by the four LHC experiments (ALICE, ATLAS, CMS, LHCb). The
numbers shown represent the WLCG resources from 2022.}
\label{fig:wlcg}
\end{center}
\end{figure}

These software elements are in constant use, as computing operations
continues 24 hours a day, 7 days a week throughout the year.
The LHC experiments rely on
$\sim$170 computing centers and national grid infrastructures that
are federated via the Worldwide LHC Computing Grid (shown in
Figure~\ref{fig:wlcg}). The U.S.\ contribution is organized and run
by the Open Science Grid (OSG)~\cite{OSGPAPER,OSGWEB}. The intrinsic
nature of data-intensive collider physics maps very well to the use
of high-throughput computing. The computing use ranges from
``production'' activities that are organized centrally by the
experiment (e.g., basic processing of RAW data from the detector and 
creation of high statistics Monte Carlo simulations) to ``analysis'' activities 
initiated by individuals or small groups of researchers for their specific
research investigations.

\vskip 0.1cm
\noindent{\bf Software Stacks:} In practice much of the actual software and 
infrastructure is implemented {\em independently} by each experiment. This 
includes managing 
the software development and deployment process and the resulting software
stack. Some of this is a natural result of the intrinsic differences
in the actual detectors (scientific instruments) used by each experiment.
Independent software stacks are also the healthy result of
different experiments and groups making independent scientific investigations 
using different algorithmic and 
implementation choices. And last, but not least, each experiment must
have control over its own schedule to insure that it can deliver physics 
results in a competitive environment. This implies sufficient control over 
the software development process and the software itself that the experiment 
uses.

The independence of the software processes in each experiment of course
has some downsides. At times, similar functionalities are implemented
redundantly in multiple experiments, parts as a by-product of the 
physics research program (i.e.\ the result of R\&D by postdocs and graduate 
students). Typically, software is developed and used without with the explicit aim of producing 
sustainable software over the lifetime of an experimental program. Issues of long term software 
sustainability can arise in these cases when the particular functionality is 
not actually mission-critical or specific to the experiment. 
%Obtaining
%human resources (both in terms of effort and in terms of intellectual
%input) can be difficult if the result only impacts one particular HEP
%experiment. \langenote{this previous thought comes from no where - so far everything 
%has been in the context of a single experiment ``owning'' its manpower. I would drop the sentence}
Trivial technical and/or communication issues can prevent
even high quality tools developed in one experiment from being adopted
by another.

The HEP community has nonetheless a developed an ecosystem of common software 
tools that are widely shared in the community. Ideas and experience
with software and computing in the HEP community are shared at 
general dedicated HEP software/computing conferences such as 
the Conference on Computing in High Energy and Nuclear Physics (CHEP)~\cite{CHEP2016},
the Workshop on Advanced Computing and Analysis Techniques (ACAT)~\cite{ACAT2017} and HEPiX~\cite{HEPiX}. 
In addition there are many 
specialized workshops on software and techniques for pattern recognition, 
simulation, data acquisition, use of machine learning, and other 
topics.

An important exception to the organization of software stacks 
by the experiments is the national grid infrastructures, such as the OSG
in the U.S. The federation of computing resources from
separate computing centers which at times support more than one HEP experiment 
or that support HEP and other scientific domains requires and creates
incentives that drive the development and deployment of ``common'' 
solutions.

%  The community also a long history with ``common software'' projects. 
%Despite the best of intentions many of these projects are seen as having
%failed to deliver XXXX   

%\vskip 0.1cm
%\noindent{\bf Application Software Examples:} More than 10M lines of code 
%%mentioned earlier that 
%have been developed within individual experiments to implement the relevant
%data acquisition, data handling, pattern recognition and processing, 
%calibration, simulation and analysis algorithms. These code bases also include 
%application frameworks, data persistence and related support 
%libraries needed to structure the myriad of algorithms into single data 
%processing applications. 
%Much of the code is experiment-specific due to 
%real differences in the detectors used by each experiment and the techniques
%appropriate to the different instruments. Some code is however simply 
%redundant development of different implementations of the same 
%functionalities. 
%This code base contains significant portions which are a by-product of the 
%physics research program (i.e. the result of R\&D by postdocs and graduate 
%students) and typically without with the explicit aim of producing 
%sustainable software. Long term
%sustainability issues exist in many places in such code. One obvious
%example is the need to develop parallel algorithms and implementations for the
%increasingly computationally intensive charged particle track reconstruction.
%%A challenge for the Institute will be to forge
%%effective collaborative efforts between the experiments to solve the
%%software issues.

\vskip 0.1cm
\noindent{\bf Examples of Shared Application Software Toolkits:}
The preparations for the LHC have nonetheless yielded important community 
software tools for data analysis like ROOT~\cite{root} and detector simulation
Geant4~\cite{Geant4Ref1,Geant4Ref2,Geant4Ref3}, both of which have been
critical not only for LHC but in most other areas of HEP and beyond.
Other tools have been shared between some, but not all, experiments.
Examples include
the GAUDI~\cite{GAUDI} event processing framework,
IgProf~\cite{IGPROF} for profiling very large C++ applications like those used
in HEP, 
RooFit~\cite{Verkerke:2003ir} for data modeling and fitting and
the TMVA~\cite{Hocker:2007ht} toolkit for multivariate data analysis.

In addition software is a critical tool for the interaction and knowledge
transfer between experimentalists and theorists. 
Software provide an important physics input from the theory community to 
the LHC experimental program, for example through event 
generators such
as SHERPA~\cite{SHERPA} and ALPGEN~\cite{ALPGEN} and through jet finding 
tools like FastJet~\cite{FASTJET1,FASTJET2}, which is a critical piece of 
software for the LHC experiments RAW data processing applications.

%This is not meant to be an exhaustive list. 
%The Community White Paper provides a more complete software
%development roadmap, along with potential solutions to the
%sustainability challenges for each software package 
%and relevance to the long-run HL-LHC and broader  HEP programs.

\vskip 0.1cm
\noindent{\bf Infrastructure Software Examples:} 
As noted above, the need for reliable ``infrastructure'' tools which must 
be deployed as services in multiple computer centers creates incentives for the 
development of common tools which can be used by multiple HEP experiments,
and often by other scientific applications.
Examples include
%developed in collaboration with computer scientists include
FRONTIER~\cite{FRONTIER} for cached access to databases,
XROOTD~\cite{XROOTD} and dCache~\cite{DCACHE} for distributed access to
bulk file data, 
Rucio~\cite{RUCIO} for distributed data management,
EOS~\cite{EOS1,EOS2} for distributed disk storage cluster 
management,
FTS~\cite{FTS} for data movement across the distributed computing system,
CERNVM-FS~\cite{CERNVMFS} for distributed and cached access to software,
GlideinWMS~\cite{GLIDEINWMS} and PanDA~\cite{PANDA1,PANDA2} for
workload management. 
Although not developed specifically for HEP, HEP has been an important
domain-side partner in the development of tools such as 
HTCondor~\cite{condor-practice} for distributed high throughput computing 
and the Parrot~\cite{PARROT} virtual file system.

Global scientific collaborations need to meet and discuss, and this has 
driven the development of the scalable event organization software 
Indico~\cite{INDICO1,INDICO2}.  Various tools have been developed by
the HEP community to support information exchange and preservation across
the experimental and theoretical communities. Examples include: the
preservation of experimental data samples, analysis results, 
and software developed by experiments (e.g., RECAST~\cite{Cranmer2011} and REANA~\cite{reanaweb}); 
information discovery for HEP papers, authors, and collaborations (e.g., INSPIRE~\cite{inspireweb}); 
and to facilitating technical collaborations (e.g, SWAN analysis service based on 
notebook technologies~\cite{swan}).

In a similar way, the CS and HEP communities have collaborated on the
broader problems of data and software
preservation such as the DASPOS Project~\cite{daspos-project} in
scientific computing, which has led to case studies and software
prototypes applied to LHC software as well as service prototypes such
as the CERN data analysis portal.

\subsection{Software Development and Processes in the HEP Community}
\label{sec:hepsw}
The HEP community has by necessity developed significant experience in 
creating software infrastructure and processes that integrate 
contributions from large, distributed communities of physics researchers. 
To build its software ecosystem, each of the major 
HEP experiments provides a set of
``software architectures and lifecycle processes, development,
testing and deployment methodologies, validation and verification
processes, end usability and interface considerations, and required
infrastructure and technologies'' (to quote the NSF \s2i2 solicitation~\cite{NSF15553}).
Computing hardware to support the development process for the application
software (such as continuous integration, development, and test machines) 
is typically provided by the host laboratory of each experiment, 
e.g., CERN for the LHC experiments. Each experiment
manages software release cycles for its own unique application software code
base, and works to update software elements, such has shared software toolkits,
 that are integrated into its software stack. Release cycles are organized 
to meet goals ranging from physics needs, to bug and performance fixes. The 
software development infrastructure is also designed to allow 
individuals to write, test and contribute software from any laboratory, university,
or personal laptop.  The software development and testing support for 
the ``infrastructure'' part of the software ecosystem, supporting the 
distributed computing environment, is more diverse and not centralized at 
CERN. It relies much more heavily on resources such as the Tier-2 centers 
and the OSG. Given the non-uniformity in computing site infrastructures, 
the integration and testing process for computing infrastructure software elements 
is complex than that for application software. Nevertheless, the 
full set of processes has also been put in place by each LHC experiment, and continues to evolve
as the software stacks change.

%\begin{figure}[htbp]
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.96\textwidth]{images/cmssw-authors-per-month.png}
\caption{Evolution of the number of individuals making contributions to the CMS application software release each month over the period from 2007 to 2016. Also shown is how the
developer community was maintained through large changes to the technical
infrastructure, in this case the evolution of the version control system from 
CVS hosted at CERN to git hosted in GitHub. This plot shows only the application software managed in the experiment-wide software release (CMSSW) and not ``infrastructure'' software (e.g., for data and workflow management) or ``analysis'' software developed by individuals or small groups.
\label{fig:cmsswdevelopers}}
\end{center}
\end{figure}

For the most part, the HEP community has not 
formally adopted any explicit development methodology or model, however the 
de-facto method adopted is very similar to agile software 
development~\cite{AGILE}.
On slightly longer time scales, the software development
efforts within the experiments must respond to various
challenges including evolving physics goals and discoveries, general
infrastructure and technology evolution, as well as the evolution of the
experiments themselves (detector upgrades, accelerator energy, and
luminosity increases, etc.). 
HEP experiments have also maintained these software infrastructures
over time scales ranging from years to decades and in projects
involving hundreds to thousands of developers. 
Figure~\ref{fig:cmsswdevelopers} shows the example
of the application software release (CMSSW) of CMS experiment at the LHC. 
Over a ten year period, up to
300 people were involved in making changes to the software each month.  
The software process shown in the figure results in the integration, testing 
and deployment of tens of releases per year on the global computing 
infrastructure. 
The figure also shows an example of the evolution in the
technical infrastructure, in which the code version control system was
changed from CVS (hosted at CERN) to git (hosted on GitHub~\cite{cmsswgithub}). 
Similar software processes are also in routine
use to develop, integrate, test and deploy the computing infrastructure 
elements in the software ecosystem which support distributed data management
and high throughput computing.

In this section, we described ways in which HEP community develops
its software and manages its computing environment to produce physics
results. In the next section (Section~\ref{sec:role}), we present the
role of the Institute to facilitate a successful HL-LHC physics program
through targeted software development and leadership, more generally,
within the HEP software ecosystem.




\tempnewpage


==> 999-todo-list.tex <==
\section{Appendix - TODO list for the Strategic Plan writeup}
\label{todolist}

This is a list of smaller things to do to finalize the Strategic Plan:

\begin{itemize}
\item AAA
\item BBB
\item CCC
\end{itemize}

